A Comparative Study between HLS and HDL on SoC for Image Processing Applications

The increasing complexity in today's systems and the limited market times demand new development tools for FPGA. Currently, in addition to traditional hardware description languages (HDLs), there are high-level synthesis (HLS) tools that increase the abstraction level in system development. Despite the greater simplicity of design and testing, HLS has some drawbacks in describing harware. This paper presents a comparative study between HLS and HDL for FPGA, using a Sobel filter as a case study in the image processing field. The results show that the HDL implementation is slightly better than the HLS version considering resource usage and response time. However, the programming effort required in the HDL solution is significantly larger than in the HLS counterpart.

==> relworks_v1.tex <==
\subsection{Related Works}
 
 In the literature, there are numerous works that propose HLS or HDL solutions to different problems. However, just a few implement the same algorithm with both HLS and HDL.
%Para comparar las implementaciones hardware en FPGA diseñadas con HDL respecto de los HLL, la comunidad científica ha realizado numerosas investigaciones. 
En general, los resultados obtenidos en los estudios demuestran que HLL  disminuye los tiempos de desarrollo por el nivel de abstracción mayor y la “familiaridad” de los diseñadores con los lenguajes de este tipo. Sin embargo, los HDL suelen emplear los recursos de las FPGA de mejor manera y obtienen velocidades mayores de operación en los diseños. 

Las afirmaciones anteriores apoyan una corriente de pensamiento que anticipa un reemplazo de HLL respecto a HDL en FPGA. Entre las investigaciones que están alineadas con estas afirmaciones, se encuentran diversos estudios comparativos en el ámbito de visión en tiempo real~\cite{hiraiwa_fpga_2013,tetrault_two_2018}, de la compresión de video~\cite{pelcat_design_2016}, del procesamiento de imágenes~\cite{zwagerman_high_2015,gurel_computer_nodate}, del álgebra abstracta~\cite{stanciu_comparison_2017}, o de las finanzas~\cite{stamoulias_hardware_2017}.

En sentido contrario a las investigaciones anteriores, un estudio reciente en el ámbito de la inteligencia artificial demostró que HDL podría resultar superior para desarrollar diseños parametrizables respecto de HLL, cuando el diseño tiene características particulares~\cite{aledo_vhdl_2019}. %Empleando como caso de estudio una red de neuronas artificiales, los autores determinaron que HDL dispone de herramientas más potentes respecto a HLL para obtener diseños genéricos que sean altamente parametrizables, lo que eleva el costo de programación del segundo. 
Este trabajo permite suponer que los HDL podrían ser una mejor opción para algunos desarrollos, o partes de ellos, respecto a HLL.% al utilizar sentencias genéricas. 

En general, las comparaciones entre HLL y HDL en FPGA parecen concluir de forma similar en lo que refiere al costo de programación. Hasta donde llega el conocimiento del tesista, el uso de HLL respecto a HDL está en aumento, ya que los tiempos menores de desarrollo en alto nivel permiten hacer frente a los exigentes tiempos de mercado. Sin embargo, no hay tendencias claras en lo que refiere al rendimiento y el uso de recursos por parte de cada uno de estos dos enfoques, estando fuertemente influenciados por las características del problema a resolver.
FALTA: En este trabajo se busca ide
